P$^{2}$Net: Patch-match and Plane-regularization for Unsupervised Indoor Depth Estimation

This paper tackles the unsupervised depth estimation task in indoor environments. The task is extremely challenging because of the vast areas of non-texture regions in these scenes. These areas could overwhelm the optimization process in the commonly used unsupervised depth estimation framework proposed for outdoor environments. However, even when those regions are masked out, the performance is still unsatisfactory. In this paper, we argue that the poor performance suffers from the non-discriminative point-based matching. To this end, we propose P$^2$Net. We first extract points with large local gradients and adopt patches centered at each point as its representation. Multiview consistency loss is then defined over patches. This operation significantly improves the robustness of the network training. Furthermore, because those textureless regions in indoor scenes (e.g., wall, floor, roof, \etc) usually correspond to planar regions, we propose to leverage superpixels as a plane prior. We enforce the predicted depth to be well fitted by a plane within each superpixel. Extensive experiments on NYUv2 and ScanNet show that our P$^2$Net outperforms existing approaches by a large margin. Code is available at \url{https://github.com/svip-lab/Indoor-SfMLearner}.

==> sections/tmp.tex <==
Depth estimation is a fundamental part in vision research, bridging the gap between 2D images and 3D world.  Lots of supervised depth estimation frameworks \cite{fu2018deep} \cite{liu2015learning}  are proposed with the recent trend in convolution neural networks (CNNs). However, capturing a large amount of images with accurate ground truth depth can be time-consuming and expensive. To overcome the above challenge, another line of work focus on unsupervised depth estimation that based on purely videos and known camera intrinsic as input.

Interestingly, the same training process can easily collapse on indoor datasets, i.e, predicted depth being infinite and pose being identity in the first few epochs. Similar problems \cite{godard2019digging}\cite{luo2018every} are also observed on typical outdoor datasets when there exist objects that are moving with the same velocity as the camera. This can be attributed to the projective camera model. \TODO{samespeed=objects at infinite depth}. While the amount of such regions can be small on outdoor datasets, the large non-texture regions on indoor datasets can easily overwhelm the training process. In this paper, we propose a masking process which filters out easy stationary points to bootstrap the network and avoid the aforementioned trivial solutions. Specifically, inspired from Direct Sparse Odometry(DSO) \cite{engel2017direct}, we generate key points for each image to mask out non-texture regions. Different from Moving Indoor \cite{zhou2019moving}  which requires establishing correspondences between consecutive frames, our method requires no matching process and is hence direct. To allow the flow of gradients to adjacent regions, we assume a fixed depth within a local window around these key points and leverage such patterns during the warping process. However, some non-texture regions still may not receive any supervision in the above process. We further incorporate superpixels to enforce the consistency of the predicted depth within each superpixel.

Another challenge can be the large variation of the relative pose between neighboring frames on indoor datasets with handheld cameras. We propose a simple modification to the input of the pose network that results in a better convergence.

Overall, our contribution can be summarized as follows: i) A simple modification to the pose network that allows a better convergence. ii) We generate key points to filter out textureless regions and integrate a local pattern into our warping process. %which assumes a fixed depth within a local window to allow for a larger flow of the gradient. 
iii) We combine superpixels into our network and regularize the consistency within each superpixel. Experiments on NYUv2 \cite{nyu} and Scannet \cite{dai2017scannet} datasets demonstrate that our approach achieves state-of-the-art.

